Self-Detoxifying Language Models via Toxification Reversal

Language model detoxification aims to minimize the risk of generating offensive or harmful content in pretrained language models (PLMs) for safer deployment. Existing methods can be roughly categorized as finetuning-based and decoding-based. However, the former is often resource-intensive, while the latter relies on additional components and potentially compromises the generation fluency. In this paper, we propose a more lightweight approach that enables the PLM itself to achieve "self-detoxification". Our method is built upon the observation that prepending a negative steering prompt can effectively induce PLMs to generate toxic content. At the same time, we are inspired by the recent research in the interpretability field, which formulates the evolving contextualized representations within the PLM as an information stream facilitated by the attention layers. Drawing on this idea, we devise a method to identify the toxification direction from the normal generation process to the one prompted with the negative prefix, and then steer the generation to the reversed direction by manipulating the information movement within the attention layers. Experimental results show that our approach, without any fine-tuning or extra components, can achieve comparable performance with state-of-the-art methods.

==> sections/experiments_backup.tex <==


\section{Experiments}

\subsection{Experimental Setup}

\input{sections/table_auto}

%To assess the toxicity of the content generated by language models, 
\paragraph{Datasets} We use the RealToxicityPrompts~\citep{gehman-etal-2020-realtoxicityprompts} (RTP) dataset for experiments. The RTP dataset contains 100K text paragraphs extracted from English web text, with the first half of each paragraph used as a prompt and the corresponding second half as a continuation. \red{The Perspective API~\footnote{https://perspectiveapi.com} is used to score the probability of toxic content in all prompts and continuations.} We randomly sampled 10K prompts for evaluation. After excluding invalid samples, there are a total of 7,785 non-toxic prompts (score $<0.5$) and 2,122 toxic prompts (score $>0.5$), which serve as two evaluation settings. Conditioned on each prompt, LMs need to generate a minimum of 5 and a maximum of 20 tokens as continuations for evaluation. 

\paragraph{Baselines}

\paragraph{Implementation Details} We use nucleus sampling~\citep{Holtzman2020The} with p = 0.9 to sample 25 continuations for each prompt. \red{We use $\alpha=0.4$ and $\beta=0.6$ for the subsequent experiments. The values are selected via running around $\alpha \in \{0.4,0.5,0.6,0.8\}$ and $\beta \in \{0.2, 0.4,\cdots,1.6\}$, aimming for a trade-off between toxicity reduction and fluency. Full results of adjusting $\alpha$ and $\beta$, as well as whether renormalizing the modified vectors are shown in Appendix~\ref{sec:appendix_hpm}. [Comment\_by\_CY: write some more implementation details if possible]}

\subsection{Automatic Evaluation}

We adopt the experimental setup from previous work~\citep{liu-etal-2021-dexperts}, employing two evaluation metrics: Expected Maximum Toxicity and Toxicity Probability. Expected Maximum Toxicity computes the average of the highest toxicity scores across the 25 samples for a specific prompt, taking into account all prompts. Toxicity Probability, on the other hand, represents the likelihood of generating a continuation with a toxicity score of 0.5 or greater at least once within the 25 samples. Furthermore, we utilize a larger pre-trained language model, GPT2-XL~\footnote{https://huggingface.co/gpt2-xl}, to assess the fluency of the generated text by measuring its perplexity. Also, the diversity of generations, specifically the distinctiveness of 1-gram and 2-gram, is also taken into consideration in the evaluation. 

We did not use the Perspective API to assess the toxicity of newly generated text due to its limitations on request throughput. Instead, we trained an offline toxicity scorer on nearly 90k RTP samples not used for evaluation to improve efficiency. Specifically, we fine-tuned a DeBERTa-v3-large~\footnote{https://huggingface.co/microsoft/deberta-v3-large}~\citep{he2023debertav} model to fit the original API's toxicity probabilities by minimizing the KL divergence. This fine-tuned model achieved 94.87\% accuracy and a 98.54\% AUROC score on the hold-out 10k subset, which indicates that it can effectively estimate text toxicity as a substitute for the API. With this accurate estimation performance guarantee, the model has a much higher throughput than the API, i.e., ~27,000 samples per second versus typically 25 queries per second using the API.


\subsection{Human Evaluation}

We conducted a human evaluation by performing pairwise comparisons of various aspects of continuations. We randomly selected 50 prompt-continuation pairs from our approach, as well as from DAPT, \textsc{DExperts}, and SD, to determine which model produces superior continuations under the same prompt. We invite three expert annotators to assess the continuations based on toxicity, fluency, and consistency with the given prompt, and to select the better generation.



% human evaluation

\subsection{Baselines}


\paragraph{Retraining-based} The retraining-based method detoxifies the Language Model (LM) by fine-tuning it on a non-toxic dataset. We adopted two Retraining-based methods as baselines, i.e., Domain-Adaptive Pretraining (DAPT)~\citep{gururangan-etal-2020-dont} and Attribute Conditioning (\textsc{AtCon})~\citep{keskar2019ctrl}. DAPT further pretrained the base LM on the non-toxic subset of OpenWebText~\citep{Gokaslan2019OpenWeb}. We used the checkpoint fine-tuned by \citet{liu-etal-2021-dexperts}. \textsc{AtCon} fine-tuned LM using control code prefixes (e.g., <|toxic|>, <|nontoxic|>). During inference, <|nontoxic|> was added to the prompts to generate non-toxic continuations. In our experiments, we utilized the outputs of \textsc{AtCon} provided by \citet{gehman-etal-2020-realtoxicityprompts}.

\paragraph{Decoding-based} The decoding-based method aims to detoxify LM during inference by suppressing the probability of potential toxic tokens. Although updating the base model's parameters is not required, maintaining fluency in the generated text and achieving better detoxification effects still necessitate training an additional guiding module or fine-tuning another language model. For comparison, we selected two representative decoding-based methods, i.e., GeDi~\citep{krause-etal-2021-gedi-generative} and \textsc{DExperts}~\citep{liu-etal-2021-dexperts}.

GeDi employed a language model conditioned on class (similar to \textsc{AtCon}) to derive classification likelihoods for every potential subsequent token using Bayes' theorem, while \textsc{DExperts} integrated the original LM with two distinct LMs, including the toxic LM known as the "anti-expert", and the non-toxic LM referred to as the "expert". The intention behind this combination was to promote tokens considered likely by the experts and unlikely by the anti-experts. For both methods, we used the models' weights released by the authors.

\paragraph{Prompt-based} The prompt-based approach leverages the inherent knowledge of toxicity in LM by employing prompts for detoxification. The Self-Debiasing (SD)~\citep{10.1162/tacl_a_00434} method entailed adding a negative prefix to the input text, guiding the model to generate toxic content. Then, by re-inputting the text without the prefix for standard generation, the method suppressed tokens with a higher probability from the initial generation, which are more likely to be toxic tokens. 

Our approach is also a prompted-based method, as it similarly uses prefixes for detoxification off-the-shelf, like SD. To ensure a fair comparison, we used the same negative prefix as in our proposed method for SD. Further discussion on prefixes can be found in Appendix~\ref{sec:appendix_prefix}. 


\subsection{Results}

The automatic evaluation results of different detoxification methods on the RTP dataset are presented in Table~\ref{tb:auto}. It is clearly demonstrated that our method significantly reduces the toxicity of continuations conditioned on both Non-Toxic and Toxic prompts with the baseline models. In addition, compared to other prompt-based methods, our method exhibits the lowest values for both the expected maximum toxicity and toxicity probability metrics, while also having the best perplexity. When compared to the methods that require additional training, our method outperforms most methods in terms of toxicity reduction and fluency maintenance on the non-toxic prompt group, and has comparable performance to the state-of-the-art method \textsc{DExperts}.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{assets/human_eval.pdf}
%     \caption{Results of human evaluation for detoxification.}
%     \label{fig:human_eval}
% \end{figure}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table}[t]
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cc|cc|cc}
\toprule[2pt]
\multirow{2}{*}{\textbf{Ours vs.}} & \multicolumn{2}{c|}{\textbf{DAPT}} & \multicolumn{2}{c|}{\textbf{\textsc{DExperts}}} & \multicolumn{2}{c}{\textbf{SD}} \\
                   & \textbf{Win}  & \textbf{Lose} & \textbf{Win}  & \textbf{Lose} & \textbf{Win}  & \textbf{Lose} \\ \hline
\textbf{Toxicity}  & \textbf{26.8} & 9.7           & \textbf{18.8} & 9.4           & \textbf{25.6} & 10.1          \\
\textbf{Fluency}   & 17.1          & \textbf{17.9} & \textbf{23.1} & 14.5          & \textbf{38.8} & 14.7          \\
\textbf{Coherence} & \textbf{26}   & 22.8          & \textbf{26.5} & 17.9          & \textbf{52.7} & 18.6          \\ \hline
\textbf{Overall}   & \textbf{23.3} & 16.8          & \textbf{22.8} & 14.0          & \textbf{39.0} & 14.5          \\ \bottomrule[2pt]
\end{tabular}
}
\caption{Results of human evaluation for detoxification (\%). Ties are not shown.}
\label{fig:human_eval}
\end{table}

Moreover, the human evaluation results shown in Figure~\ref{fig:human_eval} suggest that our method is superior to SD, which is also a prompted-based method, in terms of Toxity, Fluency, and Coherence. When comparing with DAPT and \textsc{DExperts}, the text generated by our method is considered slightly better in toxicity, while being comparable in Fluency and Coherence. We report a Fleiss's Kappa of $\kappa=0.244$. It indicates a fair agreement $(0.21<\kappa<0.40)$ among human annotators.

==> sections/introduction_backup.tex <==


\section{Introduction}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{assets/intro_fig.pdf}
    \caption{Example image caption}
    \label{fig:intro}
\end{figure}

In recent years, generative language models have demonstrated remarkable performance across a wide range of applications. However, due to the presence of toxic and biased content in their training data, these models are prone to generating harmful text when deployed \cite{kumar2023language}. To mitigate this issue, several detoxification methods have been proposed. One common approach is to fine-tune pretrained models on non-toxic data \cite{gururangan-etal-2020-dont, wang2022exploring} or align them with human preferences to promote polite behavior \cite{NEURIPS2022_b1efde53, korbak2023pretraining}. While these methods have proven effective, updating all parameters of a model can be resource-intensive, particularly with the growing trend of larger models, and may negatively impact generalization for downstream tasks.

Instead of fine-tuning, some researchers have explored detoxifying model outputs during the decoding process. This approach requires a classifier trained to estimate the probability of generated text being toxic or non-toxic \cite{Dathathri2020Plug} or relies on another language model specifically tuned for this purpose \cite{liu-etal-2021-dexperts, krause-etal-2021-gedi-generative}. The additional models are used to modify the distribution of the original, untuned language model by assigning lower probabilities to tokens that may result in toxic content. However, directly altering the original output probability can lead to a decrease in fluency \cite{xu-etal-2021-detoxifying}.

In this paper, we propose a novel detoxification method for pretrained language models that neither requires an additional tuned model nor explicitly modifies the original model's predictions. Our approach effectively detoxifies a pretrained language model without updating its parameters or fine-tuning auxiliary modules, while preserving the fluency of generated text. We draw inspiration from the observation that appending a toxic prompt at the beginning of a given text can induce a model to generate toxic content. In transformer-based language models, this negative contextualization (i.e., toxification) is facilitated by the attention mechanism. Building on this insight, we devise a reverse toxification (i.e., detoxification) process that modifies the operations within the attention mechanism, enabling detoxification while allowing the model to generate its own probability distribution.

Concretely, our method involves two inference pass steps, namely \textbf{Head-wise Toxification Direction Discovery} and \textbf{Adaptive Head-wise Detoxification}. First, we insert a prefix that describes the text as containing toxic properties in front of the context prompt, resulting in a new prompt text with a negative prefix. Similarly, we can obtain a positive prompt text. Then, we perform a batch of next token prediction inference on these two texts. During this process, we can obtain the contextually embedded value vector aggregated by each attention head at each layer. We obtain the difference vector between the value vectors when inserting the negative and positive prefixes by subtraction. This vector reflects the trend of each attention head to generate toxic text from the context. We reverse this trend to obtain an anti-toxic trend, which is used to update the corresponding head output value vector when no prefix is inserted, thereby achieving the effect of removing toxicity. 


==> sections/method_backup.tex <==


\section{Detoxification via Toxification Reversing}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=\textwidth]{assets/method_fig.pdf}
    \caption{Overview of our proposed \textbf{Toxification Reversing}. Our approach involves two forward passes for generating each new token, which first toxify the model and then reverses this toxification. In the first forward pass, we concatenate a Negative and Positive Prefix to the Context Prompt and input it into the model, using \textbf{Toxification Direction Discovery} to find the toxification direction of each attention head. In the second forward pass, we only input the Context Prompt and use \textbf{Adaptive Toxification Reversing} in each attention head to detoxify the last token's value vector. Our method allows the attention to contextualize the token representation towards detoxification as much as possible, enabling subsequent modules to receive detoxified representations and avoiding direct modification of the model's output.}
    \label{fig:method}
\end{figure*}

Given a context prompt for continuation, a LM first converts is into a sequence of $N$ tokens $T = \left\{t_1, t_2, \dots, t_N\right\}$. Each token is then embedded to a vector $\xx^0_i \in \R^d$ using an embedding matrix $E\in \R^{\lvert \V\rvert \times d}$ with vocabulary size $\lvert \V\rvert$ and fused with position embeddings via summation. The input embeddings go through a sequence of $L$ transformer layers. Each layer performs read-write processes, namely multi-head self-attention (MHSA) and MLP computation, over a residual stream. The residual stream is initially the input embeddings $\xx^0$ before getting into the first layer. 

For the MHSA sub-layer at layer $l$, it contains three projection matrices $W^\ell_Q,W^\ell_K,W^\ell_V \in \R^{d \times d}$ and one output matrix $W^\ell_O \in \R^{d \times d}$. Following \citet{elhage2021mathematical}, the columns of each projection matrix and the rows of the output matrix can be split into $H$ equal parts, corresponding to the number of attention heads $W^{\ell,h}_Q,W^{\ell,h}_K,W^{\ell,h}_V \in \R^{d \times \frac{d}{H}}$ and $W^{\ell,h}_O \in \R^{\frac{d}{H} \times d}$ for $h \in \left[1, H\right]$. The $h$-th attention head first compute the attention matrix $A^{\ell,h}\in \R^{N\times N}$ as follow:
\begin{align}
    A^{\ell,h} = \varphi\paren{
    \frac{
        \paren{\xx^{\ell-1} W^{\ell,h}_Q}
        \paren{\xx^{\ell-1} W^{\ell,h}_K}^{T}
    }
    {\sqrt{d/H}}
    +M^{\ell,h}
    },
\end{align}
where $\varphi$ is a row-wise softmax normalization and $M^{\ell,h}$ is mask that makes $A^{\ell,h}$ a lower triangular matrix. Afterwards, the output of MHSA can be computed by a sum of matrices given by different attention heads:
\begin{align}
    \label{eq:agg_value}
    \aaa^\ell &= \sum_{h=1}^H A^{\ell,h} \paren{\xx^{\ell-1}W^{\ell,h}_V} W^{\ell,h}_O \\
             &= \sum_{h=1}^H \vv^{\ell,h} W^{\ell,h}_O ,
\end{align}
where each $\vv^{\ell,h}_i \in \R^{d}$ is a contextualized value vector at position $i$. 

Subsequently, the residual stream is updated through $\xx^\ell + \aaa^\ell$. An MLP sub-layer further performs a token-wise transformation for each representation in the residual stream and updates it via summation. A layer normalization is done either after the updating\citep{ba2016layer} or before the representations are send into a sub-layer\citep{pmlr-v119-xiong20b} for distribution stabilization.

Our approach consists of two step, namely (1) \textbf{Toxification Direction Discovery} and (2) \textbf{Adaptive Toxification Reversal}.


\paragraph{Toxification Direction Discovery} Inserting a negative prefix that describes the entire text as having toxic attributes before the context prompt can greatly increase the toxicity of the generated text. The insertion can be represented as $T^{-}=[T^{-}_{\text{prefix}};T]$ with negative prefix $T^{-}_{\text{prefix}}=\left\{t_1, t_2, \dots, t_{K^-}\right\}$. Similarly, we have prompts with positive prefixes $T^{+}_{\text{prefix}}=\left\{t_{i}\right\}^{K^+}_i$ inserted, represented as $T^{+}=[T^{+}_{\text{prefix}};T]$. We denote the number of tokens of $T^{-}_{\text{prefix}}$ and $T^{+}_{\text{prefix}}$ as $N^-$ and $N^+$, respectively.

Through formula~\eqref{eq:agg_value}, we can find that this toxification process is accomplished by different attention heads. These heads add the value vector of the previous tokens to the value vector of the subsequent tokens according to the weights. The prediction of the next token involves updating the representation of the last token layer by layer to the probability distribution of the next token. Consequently, we can calculate the difference in the value vector obtained by each attention head when inserting negative and positive prefixes, respectively. This is done using the following formula:
\begin{align}
    \label{eq:toxification_vector}
    \Delta\vv^{\ell, h} = \vv^{-,\paren{\ell,h}}_{N^-} - \vv^{+,\paren{\ell,h}}_{N^+},
\end{align}
where $\vv^{-,\paren{\ell,h}}_{N^-}$ is the contextualized value vector at the last position of prompt with negative prefix, while $\vv^{+,\paren{\ell,h}}_{N^+}$ is the positive one.

\paragraph{Adaptive Toxification Reversal}
Formula \eqref{eq:toxification_vector} computes the difference between value vectors obtained from concatenated prefixes with opposing attributes (i.e., negative or positive) for each attention head. This difference effectively captures the information that the attention head extracts from the prefixes. Since the prefix attributes are opposite, the resulting difference vector represents the toxification tendency of the attention head for the current residual stream. To achieve a detoxification effect, we can utilize the opposite direction of this difference vector to guide the current value vector's update, steering it away from the toxification direction:
\begin{align}
   \vv^{\text{new},\paren{\ell, h}}_N =  \vv^{\ell, h}_N - \lambda\cdot\Delta\vv^{\ell, h},
\end{align}
where $\lambda$ controls the strength of detoxification.

To emphasize the modification effect on those attention heads which are more likely to toxify the generated text, we propose two scaling factors that make our detoxification more adaptive. As we use a difference vector that represents the direction of toxification, we can infer that the size of this vector reflects the degree of toxification brought by the corresponding head. Thus, we use the $L^2\text{-norm}$ of the difference vector to further scale the strength of modification:
\begin{align}
   \lambda_{\text{norm}} = 1+\lVert \Delta\vv^{\ell, h}\rVert_2.
\end{align}
As the negative prompt is able to toxify the generated text, which means that the representation of negative prompt is encoded with toxicity, we are able to measure the toxicity of the value vector by computing the similarity between these two vectors. This simillarity-based scaling factor can be induced as:
\begin{align}
   \lambda_{\text{sim}} = 1+\max\left\{
        0,
        \cos{
            \paren{\vv^{\ell, h}_{N}, \vv^{-,\paren{\ell, h}}_{K^-}}
        }
   \right\},
\end{align}
where $\cos{\paren{u,v}}=\frac{u\cdot v}{\lVert u\rVert_2\cdot\lVert v\rVert_2}$ is the similarity measurement, and we only further scale the modification when $\cos\paren{\cdot,\cdot}>0$. In all, the final detoxification formula follows:
\begin{align}
   \vv^{\text{new},\paren{\ell, h}}_N  = \vv^{\ell, h}_N - \lambda\cdot \lambda^\alpha_{\text{norm}} \cdot \lambda_{\text{sim}}^\beta \cdot\Delta\vv^{\ell, h},
\end{align}
where $\alpha$ and $\beta$ are two hyperparameters that control the strength of these two adaptive scaling factors.

% renormalization

To preserve the model's original capabilities as much as possible, we renormalize the updated value vectors to align with the total $L^2\text{-norm}$ of all head-wise value vectors prior to the update:
\begin{align}
   \vv^{\text{new},\paren{\ell}}_N  = \vv^{\text{new},\paren{\ell}}_N \cdot \frac{\lVert\vv^{\ell}_N\rVert_2}{\lVert\vv^{\text{new},\paren{\ell}}_N\rVert_2}.
\end{align}
This ensures that the modified value vectors remain close to the representations typically accepted by the subsequent output matrix.

